Visually Consistent Hierarchical Image Classification

Hierarchical classification predicts labels across multiple levels of a taxonomy, e.g., from coarse-level 'Bird' to mid-level 'Hummingbird' to fine-level 'Green hermit', allowing flexible recognition under varying visual conditions. It is commonly framed as multiple single-level tasks, but each level may rely on different visual cues: Distinguishing 'Bird' from 'Plant' relies on global features like feathers or leaves, while separating 'Anna's hummingbird' from 'Green hermit' requires local details such as head coloration. Prior methods improve accuracy using external semantic supervision, but such statistical learning criteria fail to ensure consistent visual grounding at test time, resulting in incorrect hierarchical classification. We propose, for the first time, to enforce internal visual consistency by aligning fine-to-coarse predictions through intra-image segmentation. Our method outperforms zero-shot CLIP and state-of-the-art baselines on hierarchical classification benchmarks, achieving both higher accuracy and more consistent predictions. It also improves internal image segmentation without requiring pixel-level annotations.

==> OLD_NeuRIPS/2-intro-old.tex <==
 
\section{Introduction}
The goal of hierarchical classification is to predict all classes at each hierarchical level simultaneously (e.g., \textit{Ruby-throated Hummingbird} - \textit{Bird}).
Figure~\ref{fig:problem} provides an example of various challenges in the hierarchical classification problem. 
For our analysis, we conduct training on the iNaturalist 2018 dataset~\citep{ref:data_iNat}, with a two-level hierarchy.
Following the most commonly used approach for hierarchical classification~\citep{chen2018fine, chang2021your, chen2022label}, we extract features from a shared backbone (ImageNet~\citep{ref:data_imagenet}-pretrained ResNet-50~\citep{ref:resnet_cvpr2016}) and train separate classifiers to predict classes at each level.
 
Unlike flat-level classification, hierarchical classification has multiple possible outputs.  The challenges arise when predictions at the fine and coarse levels differ (2nd and 3rd rows in Figure~\ref{fig:problem}). 
Even if predictions are correct at one level,  it is difficult to trust the prediction if predictions at other levels are incorrect (e.g., \textit{Ruby-throated Hummingbird} - \textit{Plant}), especially when we do not have ground truth labels at test time.
Therefore, our focus lies in achieving consistent and accurate predictions across all levels simultaneously.

However, predicting multiple levels of hierarchy is more challenging than predicting a single flat-level category, leading to a confrontation between coarse and fine level learning~\citep{chang2021your}.
That is, models trained to predict all hierarchical levels show degraded performance compared to the model trained to predict a single flat level of class.
This is because hierarchical classification entails addressing multiple classification tasks concurrently.
For instance, distinguishing between similar-looking bird species at the finest level (e.g., \textit{Anna's Hummingbird} - \textit{Ruby-throated Hummingbird}) and differentiating between birds and plants at the coarse level represent distinct tasks, each requiring attention to different regions in the image.
This phenomenon is illustrated in Figure~\ref{fig:comparison_prior}, where we observe that classifiers at each level often internally attend to different parts of the image.
From this observation, we attribute performance degradation in hierarchical recognition to the inconsistency among hierarchy classifiers. 
We seek to enhance consistency by guiding classifiers to consistently focus on the same areas, where ``\textit{bird}'' (for the coarse classifier) and ``\textit{Ruby-throated Hummingbird}'' (for the fine-level classifier) are located. 



\input{figs/intro_examples}
% \begin{figure}[t]
% \vspace{-0.6cm}
%   \begin{center}
%     \includegraphics[width=1\textwidth]{figs/problem6.png}
%   \end{center}
%   \vspace{-0.3cm}
%   \caption{\textbf{Consistency is not only necessary for hierarchical classification but also helps improve accuracy.} In hierarchical classification, categorizing all levels of classes accurately is important to establish the model's reliability. %Simultaneously learning different hierarchy levels  often leads to confrontation between classifiers at each level~\citep{chang2021your}, resulting in lower performance than learning only the single level.
%   However, training on multiple levels can lead to conflicts between classifiers, hindering performance compared to single-level training~\citep{chang2021your}.
%   % To address this challenge, we pay attention to the inconsistent cases as in the 2nd and 3rd rows, where at least one classifier could correctly identify relevant parts within the image.
%   % Our idea is that guiding classifiers at different levels to focus on the same image regions as successful ones could improve overall performance.
%   We address this challenge by focusing on inconsistent cases (like rows 2 \& 3), where some classifiers correctly identify relevant image regions. Our method encourages classifiers at all levels to consistently focus on the same image regions, potentially leveraging the correctly identified parts from one of the classifiers.
%   %focus on these successful regions, potentially improving overall accuracy.
%   %Our goal is to improve consistency so that classifiers at different levels can make consistent predictions. 
%   % In the last column, our method significantly boosts accuracy by promoting consistency between classifiers, compared to the baseline, the most common approach using separate classifiers with a shared backbone (ImageNet~\citep{ref:data_imagenet}-pretrained ResNet-50~\citep{ref:resnet_cvpr2016}) on the iNaturalist 2018 dataset~\citep{ref:data_iNat}. 
%   Compared to the baseline (separate classifiers with shared ResNet-50~\citep{ref:resnet_cvpr2016} backbone pre-trained on ImageNet~\citep{ref:data_imagenet}), by promoting consistency, our method significantly boosts accuracy on the iNaturalist 2018 dataset~\citep{ref:data_iNat}.
%   (\textcolor{mygreen}{Green} border indicates correct predictions after applying our method, and \textcolor{red}{red} indicates incorrect predictions. The outer lines represent coarse-level predictions, while the inner lines represent fine-level predictions.)
%  % \textcolor{mygreen}{$\Box$} - correct prediction at both levels, \textcolor{yellow}{$\Box$} - correct coarse level prediction, \textcolor{red}{$\Box$} - unchanged prediction after applying our method.)
%   % (Color of the box indicates change in prediction  after applying our methods: \textcolor{mygreen}{$\Box$}: correctly predicts both fine and coarse level, \textcolor{yellow}{$\Box$}: correctly predicts coarse level, \textcolor{red}{$\Box$} prediction remains unchanged.)
%   }
%   \label{fig:problem}
%    \vspace{-0.5cm}
% \end{figure}


\textbf{Our insight} is that although the fine-level classifier and the coarse classifier may have different focal points, they are inherently connected.
For instance, while the fine-level classifier examines aspects like the \textit{beak}, \textit{wings}, and \textit{feathers} to classify bird species, the coarse classifier can discern between birds and flowers by integrating these details into the overall \textit{body} of the bird.
In other words, the coarse classifier should focus on the larger part formed by grouping the features attended to by the fine classifier.
Therefore, we hypothesize that by consistently aligning the areas of focus for the fine classifier and coarse classifier, we could improve both consistency and accuracy.

To this end, we employ the recent unsupervised image segmentation method, CAST~\citep{ke2024cast}. 
CAST exhibited hierarchical segmentation, transitioning from finer to coarser segments.
CAST has demonstrated the capability to group related pixels consistently through internal parsing within images, \textit{without} segmentation labels. 
Inspired by this, we propose {\it Hierarchical-CAST} (H-CAST), which utilizes CAST to align the focus of different levels of classifiers on the same areas for hierarchical recognition.
Unlike previous hierarchical classification approaches that train separate models for each level~\citep{chang2021your, liu2022focus, chen2022label}, H-CAST is an integrated model where features learned at the fine level are grouped and passed to the coarse level (Figure~\ref{fig:comparison_prior}), ensuring \textbf{spatial consistency}.
Since our method is an integrated model, if details initially captured at the fine level are incorrect, it will receive negative signals (errors) during the learning process toward coarser levels. 
As training processes, the model is encouraged to capture accurate fine-level details to improve learning at subsequent levels. 

Additionally, we propose \ourloss to further enhance \textbf{semantic consistency} by considering label relationships across levels so that predictions at the fine-level and coarse-level align within the taxonomy.
In Figure~\ref{fig:problem}, we can observe that our method of improving consistency surprisingly leads to an enhancement in accuracy as well. 
Many previously inconsistent and incorrect cases are transformed into correct classifications.

To assess both accuracy and consistency, we evaluate our method with a new metric called Full-Path Accuracy (FPA), which measures the proportion of samples in the dataset correctly predicted at all hierarchy levels. 
Validated on common benchmarks for hierarchical recognition, our method consistently outperforms the ViT-based baseline by more than 17-25\%p in FPA metric.  We empirically demonstrate its effectiveness through extensive experimentation and analysis.  Furthermore, compared to the common segmentation learned through a flat semantic taxonomy, we demonstrate that a hierarchical semantic taxonomy also in turn improves image segmentation. 

Our key contributions can be summarized as follows.
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item \textbf{Hierarchical-CAST (H-CAST)}: We propose H-CAST to consistently align the focus of hierarchy classifiers within the image. Our model enables the utilization of various granular segments, ensuring that focus remains on the same region while fine-detailed features transitioning to broader features at the coarse level (\textbf{spatial consistency}). This expansion of the focus region fosters a natural and consistent learning process for hierarchical recognition.
    \item \textbf{\ourloss}: We introduce a novel loss function that considers label relationships across hierarchy levels (\textbf{semantic consistency}).
    Our loss enforces predictions to be correct at different levels, demanding accuracy and consistency at the same time.   
    \item These contributions combined lead to \textbf{significant improvements in both accuracy and consistency}, which we demonstrate via a new metric: Full-Path Accuracy (FPA).
\end{itemize}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figs/concept_arch.png}
%   \caption{\textbf{Comparison with prior works.} Prior works~\citep{zhu2017b, yan2015hd, liu2022focus, chen2022label, chen2018fine} train separate branches for features extracted from a shared backbone to achieve hierarchical recognition, typically connecting from coarse to fine-grained levels. In contrast, our model employs a progressive learning scheme to ensure that different hierarchical granularities contribute consistently to learning in the next level, such as learning about a bird's \textcolor{mylightred}{beak} and \textcolor{mylightred}{wings} in the finer level and then combining it in the next level to learn about bird's \textcolor{myred}{body}.}
%   \label{fig:comparison_prior}
% \end{figure}



% To learn where to focus properly, previous work designs complex attention modules~\citep{liu2022focus}.
%Therefore, our goal is to enable the model to learn the distinguishing granularity features for each level without the need for a specifically designed complex attention module to determine where to look within the image.


\input{figs/fig-example_inconsistence}
       

    






==> OLD_NeuRIPS/intro-backup.tex <==

\section{Introduction}
\input{figs/fig-problem}

Hierarchical recognition~\cite{sun2001hierarchical, dumais2000hierarchical, punera2008enhanced, giunchiglia2020coherent, chang2021your} has been a topic of interest for decades due to the inherent taxonomy present in many real-world datasets, spanning various domains such as computer vision~\cite{ref:data_imagenet, ref:data_cub200, ref:data_iNat}, natural language processing~\cite{ref:data_rcv1, ref:data_wos}, biology~\cite{ref:data_protein}, and medical research~\cite{ref:data_medical}. 
While recent computer vision research has been active in flat-level fine-grained recognition~\cite{dosovitskiy2020image, deit2021icml}, in real-world scenarios, instances often arise where object details are obscured or the resolution is poor, making predictions at the fine-grained level challenging.
For example, in an autonomous driving system, the ability to distinguish whether an object ahead is a living organism or an inanimate object at the coarse level is crucial, when precise identification at the fine-grained level is almost impossible on a rainy night.
Therefore, the hierarchical recognition problem of predicting the entire hierarchy of labels is significant. 

\input{figs/fig-example_inconsistence}

Recent hierarchical recognition methods have significantly improved accuracy by utilizing multi-branch objectives built on a shared backbone to predict classes at each level simultaneously~\cite{chang2021your, liu2022focus}. 
However, while training with separate branches can lead to high accuracy for individual classifiers, ensuring consistent predictions across different hierarchies remains challenging.
Figure~\ref{fig:comparison_prior} illustrates an example of inconsistent prediction in a two-level hierarchy using iNaturalist 2018 data~\cite{ref:data_iNat}.
In this case, we observe that while the fine-level classifier correctly identifies the ``hummingbird", the coarse-level classifier identifies the same image as a ``plant". 
We believe that the reason for such inconsistent predictions can be attributed to two main factors. 
First, the level of detail required for recognizing objects varies depending on each hierarchy level. 
For instance, at a coarse level, to distinguish between ``birds'' and ``flowers'' in an image, the model focuses on the larger objects. 
In contrast, to distinguish between a ``hummingbird'' and a ``skylark'', fine-grained level requires attention to detailed features like bird beaks, wing shapes, and feather colors.
Second, the method of using separate branches fails to fully utilize the learned information at each hierarchical level; instead, each classifier tends to focus on distinct aspects, contributing to the inconsistency in predictions.
These two factors lead to an inconsistency where bird species are well recognized at the flat level, while conspicuous large objects like plants are identified at the coarse level.


In this paper, we aim to tackle this inconsistency by training a model in a hierarchical learning process, ensuring it learns the necessary visual semantics for predicting each level consistently.
Our insight is that hierarchical levels are not distinct entities; they are part of a cohesive continuum  (\emph{e.g.,} ``Hummingbird" $\in$ ``Bird"). 
For example, if a model recognizes long and slender beaks and unique wings to distinguish hummingbirds from other birds (e.g., skylark), then at a coarse level to distinguish birds from plants, the model can recognize the bird's body by combining the previously recognized beaks and wings. 
Therefore, we argue that conducting hierarchical recognition in images should involve a \textbf{cohesive and progressive learning process}, moving \textbf{from fine-level to coarse-level} distinctions.

To this end, we propose \ourmethod to learn hierarchies consistently by adopting Vision Transformer (ViT)~\cite{dosovitskiy2020image}, with each block learning one level of the hierarchy and passing the learned information to the next level.
Furthermore, to harness the visual features of ``what" and ``where" objects are in images, we employ the recent unsupervised image segmentation method, CAST~\cite{ke2024cast}. 
CAST exhibited hierarchical segmentation during the learning phase, transitioning from finer to coarser segments.
Thus, our idea is to leverage segments of different granularities for hierarchical recognition.
Specifically, we utilize finer segments to capture fine-grained details (e.g., beaks and wings) and coarser segments for broader features (e.g., the body of a bird) at different hierarchical levels.
This approach guides the model to maintain a coherent focus on the bird's body at the coarse level, while leveraging its understanding of bird beaks and wings at the fine level to ensure ``\textbf{spatial consistency}."
Figure~\ref{fig:comparison_prior} illustrates our \ourmethod, compared with prior works training a single shared backbone alongside separate branches.

Additionally, we introduce a \ourloss to further enhance consistency by considering label relationships across levels so that predictions at the fine-level and coarse-level align within the taxonomy (``\textbf{semantic inconsistency}").
When evaluated across multiple benchmarks, our method demonstrated significant improvements in both accuracy and consistency.

We also evaluated with a new metric called All-Level Path Accuracy (ALPA), which measures the proportion of samples in the dataset correctly predicted at all hierarchy levels. 
Notably, our method outperforms the ViT-based baseline supervised with hierarchical labels by more than 10\% in ALPA metric. 
We empirically prove the effectiveness of the proposed method through extensive experiments and analysis.

Our key contributions can be summarized as follows:
\begin{itemize}
    \item \textbf{Cohesive and Progressive Learning Process}: We propose a method that facilitates a coherent and progressive learning approach in hierarchical recognition. This approach involves transitioning from fine-level to coarse-level distinctions, thereby ensuring consistent predictions across different hierarchy levels.
    \item \textbf{Utilization of Segments for Hierarchical Recognition}: Our method utilizes segments of varying granularities to improve hierarchical recognition. Finer segments are employed to capture detailed features, while coarser segments focus on broader characteristics at different hierarchy levels, thereby ensuring \textbf{spatial consistency} in predictions.
    \item \textbf{Novel Loss Function for Enhanced Consistency}: We introduce a novel loss function that considers label relationships across hierarchy levels (\textbf{semantic consistency}). 
    \item These combined learning leads to significant improvements in both accuracy and consistency, as evidenced by the All-Level Path Accuracy (ALPA) metric, demonstrating the effectiveness of our approach.
\end{itemize}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figs/concept_arch.png}
%   \caption{\textbf{Comparison with prior works.} Prior works~\cite{zhu2017b, yan2015hd, liu2022focus, chen2022label, chen2018fine} train separate branches for features extracted from a shared backbone to achieve hierarchical recognition, typically connecting from coarse to fine-grained levels. In contrast, our model employs a progressive learning scheme to ensure that different hierarchical granularities contribute consistently to learning in the next level, such as learning about a bird's \textcolor{mylightred}{beak} and \textcolor{mylightred}{wings} in the finer level and then combining it in the next level to learn about bird's \textcolor{myred}{body}.}
%   \label{fig:comparison_prior}
% \end{figure}



% To learn where to focus properly, previous work designs complex attention modules~\cite{liu2022focus}.
%Therefore, our goal is to enable the model to learn the distinguishing granularity features for each level without the need for a specifically designed complex attention module to determine where to look within the image.



       

    






\section{Introduction}


Hierarchical recognition has been a topic of interest for decades due to the inherent taxonomy present in many real-world datasets~\cite{ref:data_imagenet, ref:data_cub200, ref:data_iNat}. 
While recent research has been active in flat-level fine-grained recognition, in real-world scenarios, instances often arise where object details are obscured or the resolution is poor, making predictions at the fine-grained level challenging.
For example, in an autonomous driving system, the ability to distinguish whether an object ahead is a living organism or an inanimate object at the coarse level is crucial, even if precise identification at the fine-grained level is challenging on a rainy night.
Furthermore, as an additional advantage, hierarchical recognition serves as a means to assess the model's reliability. A situation where the fine-grained label prediction is correct but the higher-level coarse label prediction is inaccurate raises doubts about the model's trustworthiness.


Therefore, the ability to predict the entire hierarchical class simultaneously when presented with a visual image is a crucial aspect of hierarchical recognition that warrants further exploration and development.



\begin{enumerate}
    \item (Target task) The Hierarchical Fine-grained recognition - Why is hierarchical fine-grained recognition important rather than just flat-level fine-grained recognition? 
    \begin{itemize}
        \item Reason 1. Real-world data inherently possesses taxonomy, necessitating the need to predict hierarchical classes in various fields such as ecology and biology.
        \item Reason 2. When images are blurred or fine-grained details are obscured, a model capable of predicting at a coarser level, such as just ``bird" instead of a specific bird species, becomes essential. (or Autonomous driving example. Even not being able to what the fine-level object is, it should be able to predict if it's living or nonliving thing.)
        \item Reason 3. It allows for checking the reliability of the model. Even if the fine-grained label prediction is correct, if the higher-level coarse label prediction is wrong, it's difficult to trust the model's predictions. Conversely, if the fine-grained label prediction is wrong but the higher-level coarse label prediction is correct within the same parent category, it's more acceptable. 
        \item Therefore, active research has studied on hierarchical fine-grained recognition for decades [Add references]. 
        \item While traditional methods relied on tree-based algorithms to solve problems [Add references], recent advancements in deep neural networks have shown superior performance through multi-branch approaches [Add references].
    \end{itemize}
    \item (Challenges of the task that previous work could not solve: Consistency)
    \begin{itemize}
        \item However, simultaneously learning different levels is challenging, leading to a \textbf{coarse-fine tradeoff} [Refer-CVPR21:Flamingo]. That is, models trained to predict all hierarchical levels show degraded performance compared to the model trained to predict a single flat level of class.
        \item This is because the learning process of models differs depending on the level of detail they focus on within visual images [add reference]. For instance, at a coarse level, to distinguish between `birds' and `flowers' in an image, the model focuses on the larger objects. 
        In contrast, to distinguish between a `hummingbird' and a `skylark', fine-grained level requires attention to detailed features like bird beaks, wing shapes, and feather colors.
        \item Due to these distinct learning requirements, training models for multiple levels leads to (1) reduced prediction accuracy [add table/plot] and (2) inconsistencies, as in Figure~\ref{fig:example_inconsistence}.
        \item Thus, to learn where to focus properly, previous work designs complex attention modules [Liu et al., ECCV, 2022].
    \end{itemize}
    \item (Our work's motivation to solve the problem) - Inspired by CAST.
    \begin{itemize}
        \item Our goal is to train the model to learn the distinguishing granularity features for each level 
        %(without requiring additional data or specially designed module).
        \item \textbf{Our insight}: 
       In Figure 1, if the model learns details like `bird beaks' and `wing shapes' at the fine-grained level, it should focus on the `overall appearance of birds' grouped by `beaks' and `wings' at the coarse level (instead of independently focusing on a large object, such as flower). 
    \end{itemize}
    \item (Method) 
    \begin{itemize}
        \item To achieve this, we pay attention to the recent segmentation research, CAST~\cite{ke2024cast}. CAST demonstrated the ability to segment fine-to-coarse granularity using only class labels. Using this, we train the model to learn visual details (e.g., bird beaks, wings) within the image at the fine-grained level and then group these visual details learned earlier at the coarser level to learn larger parts in a consistent way (e.g., bird's body) [Todo: Visualize this segmentation]. This progressive grouping ensured internal consistency in learning. 
        \item Additionally, to further enhance consistency by considering the relationship between labels of different levels, we propose the global KL divergence loss.
    \end{itemize}
    \item (Findings) 
    \begin{itemize}
        \item Our proposed method could improve accuracy and consistency at the same time + Some interesting/surprising results. 
    \item Additional benefit: interpretabililty. 
    \end{itemize}
\end{enumerate}



\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/inconsistent_example3.png}
  \caption{[TODO finalize caption] Example of inconsistent prediction in a two-level hierarchical model. Using ResNet-50 on iNaturalist2018, the classifier correctly identified the fine-grained label as 'hummingbird,' but the coarse label was predicted as 'Plant,' resulting in an inconsistent prediction. Grad-CAM visualization of each layers show that they are attending to inconsistent regions.}
  \label{fig:example_inconsistence}
\end{figure}

In hierarchical recognition, the important and challenging task is to ensure consistent prediction across levels.
Even if the prediction is correct at the fine level, if it is incorrect at the coarser level, it will be difficult to establish the model's reliability.
Figure~\ref{fig:example_inconsistence} illustrates this example. \footnote{
Following prior works adopting multi-branch architectures, we employ a shared backbone (ResNet-50~\cite{ref:resnet_cvpr2016}) with two additional classifiers to train a 2-level hierarchy on inaturalist data~\cite{ref:data_iNat}.
}
In this case, we can observe that while the fine-level classifier correctly identifies the ``hummingbird", the coarse-level classifier identifies the same image as a ``plant". 
Notably, ``hummingbird'' and ``plant'' are not aligned within the taxonomy. 
Hence, we define such discrepancies as ``semantic inconsistency,'' where predictions at the fine-level and coarse-level are not aligned within the taxonomy.
Next, to examine where each classifier is focusing within the image, we visualize with Grad-CAM~\cite{selvaraju2017grad}.
Interestingly, the fine classifier attends to the bird, while the coarse classifier focuses on the plant.
We refer to this discrepancy where the classifiers at different levels attend to different visual regions as ``spatial inconsistency."
Our goal is  these two inconsistencies and achieving consistent predictions.



==> figs/ours_vs_cast/comparison.tex <==
\def\imw#1#2{\includegraphics[width=#2\linewidth]{#1.png}}

\def\blk#1{
\imw{figs/ours_vs_cast/imgs/#1_img_a}{0.104}\phantom{.}&
\imw{figs/ours_vs_cast/imgs/#1_seg3_flat}{0.104}\phantom{.}&
\imw{figs/ours_vs_cast/imgs/#1_seg3_hier}{0.104}
}

\def\row#1#2#3{
\blk{#1} & \blk{#2} & \blk{#3} \\[-1.5pt]
}

\begin{figure}[t]
\vspace{0pt}\centering%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
 & CAST & H-CAST &  & CAST & H-CAST &  & CAST & H-CAST \\
%\row{00000582}{00001045}{00003014}00013407
\row{00013407}{00027799}{00034086}
\row{00003014}{00013323}{00000006}
% \row{00037014}{00013363}{00024283}
% \row{00005682}{00006000}{00008780}
% \row{00003318}{00013323}{00000925}

\end{tabular}
\vspace{-3pt}
\caption{%
\textbf{Additional taxonomy information improves segmentation.} We compare our segmentation results on Entity-30 dataset with CAST at the coarsest level to explore the potential benefits of incorporating additional hierarchical label information for image segmentation. For example in the first `bird' image,  H-CAST is able to segment meaningful parts such as the face, belly, and a branch, with less fractured compared to the CAST.
Thus, H-CAST delivers an improvement in segmentation with the benefits of hierarchy. More segmentation results are shown in Appendix~\ref{appendix:sub:h_cast_vs_cast}.
}
\label{fig:cast_comparison}
\vspace{-5pt}
\end{figure}


==> figs/ours_vs_hvit/visualize_nearest.tex <==
\def\imw#1#2{\includegraphics[width=#2\linewidth]{#1.jpg}}

\def\blk#1#2{
\imw{figs/ours_vs_hvit/hvit/#1_origin}{#2}\phantom{..}&
\imw{figs/ours_vs_hvit/hvit/#1_1_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hvit/#1_2_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hvit/#1_3_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hvit/#1_4_nn}{#2}\phantom{..}&
\imw{figs/ours_vs_hvit/hcast/#1_1_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hcast/#1_2_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hcast/#1_3_nn}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hcast/#1_4_nn}{#2}\phantom{.} \\
}

\def\row#1#2{
\blk{#1}{0.099}{hvit} & \blk{#2}{0.099}{hcast} \\[-1.5pt]
}

\begin{figure}[t]
\vspace{-5mm}\centering%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\small
% & \multicolumn{3}{c}{Fine to coarse segments} &  & \multicolumn{3}{c}{Fine to coarse segments} \\
{\small Query} & {\small Rank-1} & {\small Rank-2} &{\small Rank-3}  & {\small Rank-4}& {\small Rank-1} & {\small Rank-2} & {\small Rank-3} & {\small Rank-4} \\
\blk{00000343}{0.099}
\blk{00004893}{0.099}
%\blk{00008997}{0.099}
 & \multicolumn{4}{c}{(a) Hier-ViT} & \multicolumn{4}{c}{(b) H-CAST}
\end{tabular}
\vspace{-3mm}
\caption{%
\textbf{Consistent visual grounding effectively learns an object's discriminative features.} We select the samples whose fine-grained class token features have the highest cosine similarity to the query. Hier-ViT, using only semantic supervision, retrieves visually similar but incorrect images, failing to capture class-specific features. In the top row, it ranks an image containing both a cow and a person as the second closest match to the llama query. In the bottom row, it misidentifies a small goldfinch on rocks, retrieving a dark-feathered bird with a yellow beak that shares similar overall colors but is a completely different species. In contrast, H-CAST learns more discriminative features, correctly retrieving llama and goldfinch images, even in challenging cases where Hier-ViT fails, demonstrating  the effectiveness of visual grounding. (The \textcolor{wrongred}{red border} indicates incorrect fine-grained classifications, while the \textcolor{textgreen}{green border} marks correct retrievals from the same class.)
}
\label{fig:visualize_neighbor}
%\vspace{-5mm}
\end{figure}





==> figs/ours_vs_hvit/visualize_nearest2.tex <==
\def\imw#1#2{\includegraphics[width=#2\linewidth]{#1.jpg}}

\def\blk#1#2{
\imw{figs/ours_vs_hvit/hvit/#1_origin}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hvit/#1_fine}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hvit/#1_coarse}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hcast/#1_fine}{#2}\phantom{.}&
\imw{figs/ours_vs_hvit/hcast/#1_coarse}{#2}\phantom{.}
}

\def\row#1#2{
\blk{#1}{0.094} & \blk{#2}{0.094} \\[-1.5pt]
}

\begin{figure}[t]
%\vspace{-5mm}
\centering%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\small
% & \multicolumn{3}{c}{Fine to coarse segments} &  & \multicolumn{3}{c}{Fine to coarse segments} \\
{\small Query} & {\small Fine} & {\small Coarse} &{\small Fine}  & {\small Coarse}& {\small Query} & {\small Fine} & {\small Coarse} &{\small Fine}  & {\small Coarse}\\
\row{00022684}{00003816}
\row{00046657}{00022237}
%\blk{00008997}{0.094}
 & \multicolumn{2}{c}{Hier-ViT} & \multicolumn{2}{c}{H-CAST} &
  & \multicolumn{2}{c}{Hier-ViT} & \multicolumn{2}{c}{H-CAST}\\
\end{tabular}
%\vspace{-3mm}
\caption{%
\textbf{Consistent Visual Grounding Enhances Feature Learning in Hierarchical Classification.}
We compare nearest neighbors of class token features at fine and coarse levels for queries correctly classified at both levels (Entity-30).
In the top-left,  Hier-ViT retrieves a person in a black uniform at the fine level, likely due to clothing color. This raises doubts about whether the model truly  learned the dog's  features.
%
 In the second example (top right), the query bird has gray wings with a yellow body. H-CAST retrieves a gray-winged bird at the fine level and a yellow-bodied bird at the coarse level, capturing fine-level detail and coarse-level semantics. Hier-ViT lacks this distinction.
In the final example (bottom right), the query shows two llamas  in a green field. Hier-ViT retrieves two oxen in a similar setting, resulting in fine-level misclassification. H-CAST retrieves true llama images: one showing both white and brown llamas at the fine level, and a typical llama at the coarse level.
This shows that H-CAST attends to class-relevant features while maintaining hierarchical consistency.
(\textcolor{textgreen}{Green borders} indicate same-class retrievals; \textcolor{wrongred}{red borders} indicate mismatches.)
}
\label{fig:visualize_neighbor}

\end{figure}





==> old/intro.tex <==

 
\section{Introduction} 

{Hierarchical classification~\citep{silla2011survey, chang2021your, jiang2024hierarchical} aims to predict an entire taxonomy (e.g. ``Birds''→ ``Hummingbird''→ ``Anna's hummingbird'') rather than a single-level label, making it essential for many real-world applications. The required level of detail varies by context—non-experts may only need a coarse label like \textit{Bird}, while experts such as biologists require fine-grained predictions like \textit{Anna's hummingbird}. Moreover, flat fine-grained classification often fails in ambiguous scenarios, such as when birds are viewed from a distance or in motion. In such cases, a model capable of multi-granularity predictions offers greater robustness and adaptability.

\begin{wrapfigure}{l}{0.4\textwidth} 
\captionsetup{aboveskip=2pt, belowskip=2pt} 
\vspace{-0.3cm}
\centering
\includegraphics[width=0.41\textwidth]{figs/overview.png}
\caption{\textbf{Relation to Prior Work}}
\label{fig:intro_overview}
\vspace{-0.1cm}
\end{wrapfigure}


Hierarchical classification presents several challenges, primarily because it requires recognizing objects at different levels of detail, turning it into a multitask problem. For example, the features necessary to distinguish between coarse categories (e.g., ``Birds'' vs. ``Plants'') may differ significantly from those needed to differentiate fine-grained categories (e.g., ``Green Hermit'' vs. ``Ruby-throated Hummingbird''). 
At the coarse level, the model may need broader shapes, while at the fine-grained level, it will need finer details like the bird’s beak or feather patterns.
Thus, simply applying a loss to match labels at each level can lead to conflicting optimization objectives, potentially harming fine-grained performance compared to flat classification~\citep{chang2021your}.


To address the reduced performance at the fine-grained level, state-of-the-art methods design separate blocks for each level of the hierarchy~\citep{chang2021your, chen2022label, wang2023consistency}.
While these approaches achieve good results at the fine-grained level, using separate blocks for each hierarchy level makes it difficult to resolve \textit{inconsistent} predictions — where predictions do not adhere to the hierarchical taxonomy.
Figure~\ref{fig:fig_intro} (b, c, d) shows the examples of inconsistent predictions from training FGN~\citep{chang2021your} on the 2-level hierarchy dataset, BREEDS (Entity-30)~\citep{data2021breeds}. 
For example, in the top row of image (c), the coarse classifier predicts the image as a ``motor vehicle'', while the fine-grained classifier predicts it as a ``feather boa''. %, illustrating an inconsistent prediction.
%For example, in Figure~\ref{fig:fig_intro} (c, top), there is a person wearing a feather boa on his head while riding a bicycle. 
% An ideal hierarchical model would either recognize the object on the head as a ``feather boa'' (fine-grained), and classify it as ``neckwear'' (coarse), or recognize the ``bicycle'' (fine-grained) as a ``motor vehicle'' (coarse). 
% However, FGN made inconsistent predictions, classifying the fine-grained class as ``feather boa'' while the coarse class as ``motor vehicle.''
% The alignment is essential for reliable system, as the ground-truth answers are unknown at test time, complicating trust in both coarse and fine predictions.
%
% They also model semantic relationships in the loss functions~\citep{chen2022label, wang2023consistency}, so that predictions at both the coarse and fine-grained levels align with the taxonomy.
% %primarily focusing on the \textit{semantic consistency} of taxonomy information. 
% These approaches have performed well on popular benchmarks for hierarchical classification, such as CUB~\citep{ref:data_cub200}, Aircraft~\citep{ref:data_air}, and Stanford Cars~\citep{ref:data_cars}. These datasets mainly consist of object-centric images that feature a single object, with each dataset representing only one class (e.g., birds for CUB, aircraft for Aircraft, and cars for Stanford Cars). However, real-world images often contain multiple classes in a single image, making inconsistent predictions more likely to occur.
%
%

To understand the reasons behind these inconsistencies, we use Grad-CAM visualization~\citep{selvaraju2017grad} and discover that \textbf{the coarse and fine-grained classifiers separately attend to different areas} (Figure~\ref{fig:fig_intro}, bottom). 
For instance, in case (c), the fine-grained classifier correctly attends to the part of the ``feather boa'', while the coarse classifier focuses on the bicycle's handlebars and frame,  leading to a misprediction as  ``Motor vehicle''.
%leading to the classification of the object as a motor vehicle.
%Similarly, in Figure~\ref{fig:fig_intro} (d), the model misclassifies the object as a ``primate'' by focusing on the black fur and feather in the hair at the coarse level. At the fine-grained level, it misidentifies the object as a ``shower cap'' by focusing on the forehead. 
In contrast, in the consistently correct prediction case (Figure~\ref{fig:fig_intro} (a)), the fine-grained classifier focuses on the tail and leg areas to distinguish the ``white stork'' from other bird species, while the coarse classifier captures the overall shape of the bird, including the \textit{leg area}, which the fine-grained classifier also attends to.
{This trend was frequently observed, and we provide quantitative validation in Appendix~\ref{appendix:quantitative_gradcam}.}
%From this, we newly discover that \textbf{the inconsistency in hierarchical classification arises when the coarse and fine-grained classifiers are attending to different regions of the image independently, rather than working together to recognize the same object.}

\input{figs/intro_examples}


From this observation, we argue that hierarchical classification can improve when coarse and fine-grained classifiers maintain \textbf{visual consistency, focusing on the same object at different levels of detail}. Based on this insight, we propose a novel method that align their focus areas, rather than training them as separate blocks .
%that consistent and accurate hierarchical classification can be achieved by aligning the focus areas of the fine-grained and coarse classifiers, rather than training them as separate blocks. 
This concept is illustrated in Figure~\ref{fig:comparison_prior} (right).
%\textbf{Our insight} is that although the fine-grained classifier and the coarse classifier focus on different details, they are inherently connected since both labels ultimately identify the same object.
For instance, while the fine-grained classifier examines features such as the \textit{beak}, \textit{wings}, and \textit{tail} to classify ``Green Hermit'', the coarse classifier differentiates  between ``birds'' and ``plants'' by integrating these details into the overall \textit{body} of the bird.
Therefore, we propose a new integrated model, which groups fine-grained details into increasingly coarse shapes and transfers  features learned at each hierarchy level to the next. This progressive learning scheme can effectively address inconsistencies in hierarchical classification compared to previous  methods learning each feature at an independent block.


To identify and group the visual details in an image, we employ the recent unsupervised image segmentation method, CAST~\citep{ke2024cast}.
%, since CAST exhibited hierarchical segmentation, transitioning from finer to coarser segments.
CAST has demonstrated the capability to group related pixels consistently through internal parsing within images, \textit{without} segmentation labels. 
Inspired by this, we propose {\it Hierarchical-CAST} (H-CAST), which utilizes fine-to-coarse semantic parsing to align the focus of different levels of classifiers on the same areas for hierarchical classification.
% Unlike previous hierarchical classification approaches that train separate models for each level~\citep{chang2021your, liu2022focus, chen2022label}, H-CAST is an integrated model where features learned at the fine-grained level are grouped and passed to the coarse level (Figure~\ref{fig:comparison_prior}), ensuring \textbf{spatial consistency}.
To the best of our knowledge, our work is the first to \textbf{address \textit{visual consistency} in hierarchical classification by utilizing unsupervised semantic segments}. 
Since our method is an integrated model, if details initially captured at the fine-grained level are incorrect, it will receive negative signals (errors) during the learning process toward coarser levels. 
As training processes, the model is encouraged to capture accurate fine-grained details to improve learning at subsequent levels. 

Additionally, we propose \ourloss to further enhance \textbf{\textit{semantic consistency}} by considering label relationships across levels so that predictions at the fine-grained level and coarse level align within the taxonomy.
As a result, our proposed method can achieve consistently correct predictions across all cases in Figure~\ref{fig:fig_intro}.


Firstly, we evaluate CLIP~\citep{ref:clip_2021} and show that even vision foundation models struggle with inconsistent hierarchical classification. 
Then, to assess both accuracy and consistency, we evaluate our method with a new metric called Full-Path Accuracy (FPA), which measures the proportion of samples in the dataset correctly predicted at all hierarchy levels. 
Validated on common benchmarks for hierarchical recognition, our method consistently outperforms the state-of-the-art methods with fewer parameters and training time.  We empirically demonstrate its effectiveness through extensive experiments and analysis.  Furthermore, compared to the common segmentation learned through a flat semantic taxonomy, we demonstrate that a hierarchical semantic taxonomy also in turn improves image segmentation. 

% \todo{To-do: Modification }
% Our key contributions can be summarized as follows.
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
% \item We analyze that inconsistency in hierarchical classification result from each classifiers focusing on inconsistent regions in the image. 
% %at different granularities could be fundamentally different tasks which require visual attention to same objects capturing different level of details in the image.
% \item Based on analysis, we propose \textbf{Hierarchical-CAST (H-CAST)}, an integrated hierarchical classification model with consistent visual grounding.
% \item We further propose a simple and effective Tree-path KL Divergence loss to ensure semantic consistency.
% \item Our extensive experiments on multiple benchmarks show that our H-CAST outperforms both hierarchical classification models and even flat-level models.
% Our method has been validated by substantial gains on multiple datasets, which are not trivial and not foreseeable ahead of any experimentation.
    % \item \textbf{Hierarchical-CAST (H-CAST)}: We propose H-CAST to consistently align the focus of hierarchy classifiers within the image. Our model enables the utilization of various granular segments, ensuring that focus remains on the same region while fine-detailed features transitioning to broader features at the coarse level (\textbf{spatial consistency}). This expansion of the focus region fosters a natural and consistent learning process for hierarchical recognition.
    % \item \textbf{\ourloss}: We introduce a novel loss function that considers label relationships across hierarchy levels (\textbf{semantic consistency}).
    % % Our loss enforces predictions to be correct at different levels, demanding accuracy and consistency at the same time.   
    % \item These contributions combined lead to \textbf{significant improvements in both accuracy and consistency}, which we demonstrate via a new metric: Full-Path Accuracy (FPA).
% \end{itemize}




%5. 이렇게 consistent한 visual grounding을 위해 우리는 recent work CAST 이용. 
% 이전에는 consistent visual grounding 고려한 work가 없었다는 것 강조!.

%% Summary --> 강조
%1. Our analysis reveals that classification at different granularities could be fundamentally different tasks which require visual attention to different regions in the image.
% 2. Our key insight following this revelation is that consistent visual grounding is crucial to connect hierarchical classifiers across levels.
% 3. Our computational realization of consistent visual grounding is a hierarchical classification version of CAST.  No prior research in hierarchical classification has tackled inconsistency through consistent visual grounding and the use of unsupervisedly learned segments.
% 4. Our further technical contribution is a simple and effective Tree-path KL Divergence loss to ensure semantic consistency.
% 5. Our method has been validated by substantial gains on multiple datasets, which are not trivial and not foreseeable ahead of any experimentation.

\iffalse

The goal of hierarchical classification is to predict all classes at each hierarchical level simultaneously (e.g., \textit{Ruby-throated Hummingbird} - \textit{Bird}).
Figure~\ref{fig:problem} provides an example of various challenges in the hierarchical classification problem. 
For our analysis, we conduct training on the iNaturalist 2018 dataset~\citep{ref:data_iNat}, with a two-level hierarchy.
Following the most commonly used approach for hierarchical classification~\citep{chen2018fine, chang2021your, chen2022label}, we extract features from a shared backbone (ImageNet~\citep{ref:data_imagenet}-pretrained ResNet-50~\citep{ref:resnet_cvpr2016}) and train separate classifiers to predict classes at each level.
 
Unlike flat-level classification, hierarchical classification has multiple possible outputs.  The challenges arise when predictions at the fine and coarse levels differ (2nd and 3rd rows in Figure~\ref{fig:problem}). 
Even if predictions are correct at one level,  it is difficult to trust the prediction if predictions at other levels are incorrect (e.g., \textit{Ruby-throated Hummingbird} - \textit{Plant}), especially when we do not have ground truth labels at test time.
Therefore, our focus lies in achieving consistent and accurate predictions across all levels simultaneously.

However, predicting multiple levels of hierarchy is more challenging than predicting a single flat-level category, leading to a confrontation between coarse and fine-grained level learning~\citep{chang2021your}.
That is, models trained to predict all hierarchical levels show degraded performance compared to the model trained to predict a single flat level of class.
This is because hierarchical classification entails addressing multiple classification tasks concurrently.
For instance, distinguishing between similar-looking bird species at the finest level (e.g., \textit{Anna's Hummingbird} - \textit{Ruby-throated Hummingbird}) and differentiating between birds and plants at the coarse level represent distinct tasks, each requiring attention to different regions in the image.
This phenomenon is illustrated in Figure~\ref{fig:comparison_prior}, where we observe that classifiers at each level often internally attend to different parts of the image.
From this observation, we attribute performance degradation in hierarchical recognition to the inconsistency among hierarchy classifiers. 
We seek to enhance consistency by guiding classifiers to consistently focus on the same areas, where ``\textit{bird}'' (for the coarse classifier) and ``\textit{Ruby-throated Hummingbird}'' (for the fine-level classifier) are located. 





\textbf{Our insight} is that although the fine-level classifier and the coarse classifier may have different focal points, they are inherently connected.
For instance, while the fine-level classifier examines aspects like the \textit{beak}, \textit{wings}, and \textit{feathers} to classify bird species, the coarse classifier can discern between birds and flowers by integrating these details into the overall \textit{body} of the bird.
In other words, the coarse classifier should focus on the larger part formed by grouping the features attended to by the fine classifier.
Therefore, we hypothesize that by consistently aligning the areas of focus for the fine classifier and coarse classifier, we could improve both consistency and accuracy.

To this end, we employ the recent unsupervised image segmentation method, CAST~\citep{ke2024cast}. 
%CAST exhibited hierarchical segmentation, transitioning from finer to coarser segments.
CAST has demonstrated the capability to group related pixels consistently through internal parsing within images, \textit{without} segmentation labels. 
Inspired by this, we propose {\it Hierarchical-CAST} (H-CAST), which utilizes CAST to align the focus of different levels of classifiers on the same areas for hierarchical recognition.
Unlike previous hierarchical classification approaches that train separate models for each level~\citep{chang2021your, liu2022focus, chen2022label}, H-CAST is an integrated model where features learned at the fine-grained level are grouped and passed to the coarse level (Figure~\ref{fig:comparison_prior}), ensuring \textbf{spatial consistency}.
Since our method is an integrated model, if details initially captured at the fine-grained level are incorrect, it will receive negative signals (errors) during the learning process toward coarser levels. 
As training processes, the model is encouraged to capture accurate fine-level details to improve learning at subsequent levels. 

Additionally, we propose \ourloss to further enhance \textbf{semantic consistency} by considering label relationships across levels so that predictions at the fine-level and coarse-level align within the taxonomy.
In Figure~\ref{fig:problem}, we can observe that our method of improving consistency surprisingly leads to an enhancement in accuracy as well. 
Many previously inconsistent and incorrect cases are transformed into correct classifications.

To assess both accuracy and consistency, we evaluate our method with a new metric called Full-Path Accuracy (FPA), which measures the proportion of samples in the dataset correctly predicted at all hierarchy levels. 
Validated on common benchmarks for hierarchical recognition, our method consistently outperforms the ViT-based baseline by more than 17-25\%p in FPA metric.  We empirically demonstrate its effectiveness through extensive experiments and analysis.  Furthermore, compared to the common segmentation learned through a flat semantic taxonomy, we demonstrate that a hierarchical semantic taxonomy also in turn improves image segmentation. 

Our key contributions can be summarized as follows.
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item \textbf{Hierarchical-CAST (H-CAST)}: We propose H-CAST to consistently align the focus of hierarchy classifiers within the image. Our model enables the utilization of various granular segments, ensuring that focus remains on the same region while fine-detailed features transitioning to broader features at the coarse level (\textbf{spatial consistency}). This expansion of the focus region fosters a natural and consistent learning process for hierarchical recognition.
    \item \textbf{\ourloss}: We introduce a novel loss function that considers label relationships across hierarchy levels (\textbf{semantic consistency}).
    Our loss enforces predictions to be correct at different levels, demanding accuracy and consistency at the same time.   
    \item These contributions combined lead to \textbf{significant improvements in both accuracy and consistency}, which we demonstrate via a new metric: Full-Path Accuracy (FPA).
\end{itemize}

\fi

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figs/concept_arch.png}
%   \caption{\textbf{Comparison with prior works.} Prior works~\citep{zhu2017b, yan2015hd, liu2022focus, chen2022label, chen2018fine} train separate branches for features extracted from a shared backbone to achieve hierarchical recognition, typically connecting from coarse to fine-grained levels. In contrast, our model employs a progressive learning scheme to ensure that different hierarchical granularities contribute consistently to learning in the next level, such as learning about a bird's \textcolor{mylightred}{beak} and \textcolor{mylightred}{wings} in the finer level and then combining it in the next level to learn about bird's \textcolor{myred}{body}.}
%   \label{fig:comparison_prior}
% \end{figure}



% To learn where to focus properly, previous work designs complex attention modules~\citep{liu2022focus}.
%Therefore, our goal is to enable the model to learn the distinguishing granularity features for each level without the need for a specifically designed complex attention module to determine where to look within the image.


\input{figs/fig-example_inconsistence}
       

    






==> old2-intro.tex <==

\section{Introduction} 
\vspace{-4mm}
\begin{figure}[b]
\centering  
\vspace{-5mm}
\includegraphics[width=0.8\linewidth]{figs/overview3.png}
  \caption{\textbf{We introduce internal visual consistency to align visual focus areas across levels in hierarchical semantic classification.}
Unlike single-level classification, hierarchical classification predicts labels at multiple levels of a taxonomy. When multiple objects appear in an image (\emph{e.g.}, \textit{bird} and \textit{flower}), it is important that all levels  focus on the same object to ensure semantic coherence. To encourage this, we introduce internal visual consistency, which aligns visual focus across levels.
}\label{fig:intro_overview}
\vspace{-7mm} % 필요시 조정
\caption*{
  \flushleft
  \noindent\makebox[4cm]{\hrulefill} \\ 
  {\footnotesize Code available at \url{https://github.com/pseulki/hcast}.}
}
\end{figure}

Hierarchical classification~\citep{silla2011survey, chang2021your, jiang2024hierarchical} predicts labels along a semantic taxonomy (e.g., \textit{Bird} $\rightarrow$ \textit{Hummingbird} $\rightarrow$ \textit{Green hermit}), rather than choosing from a single flat label set. This flexibility aligns well with real-world needs: a casual observer may only recognize a general category like \textit{Bird}, while a biologist might identify the exact species (Fig.~\ref{fig:intro_overview}). When visual cues are limited—such as with distant or obscured subjects—hierarchical models can still offer informative predictions, whereas flat classifiers may fail entirely.
 
%Hierarchical classification~\citep{silla2011survey, chang2021your, jiang2024hierarchical} aims to predict an entire semantic taxonomy tree (e.g. \textit{Birds}→ \textit{Hummingbird} → \textit{Green hermit}) rather than a single flat-level label, making it crucial in real-world applications (Fig.~\ref{fig:intro_overview}). The required level of detail varies by context—non-experts may only need a coarse label like \textit{Bird}, while experts such as biologists require fine-grained predictions like \textit{Green hermit}. Moreover, single-level fine-grained classification often fails in ambiguous scenarios, such as  birds  viewed from a distance or in motion.  In such cases, a model capable of full-taxonomy predictions offers greater robustness and adaptability.
% 


% \begin{wrapfigure}{l}{0.4\textwidth} 
% \captionsetup{aboveskip=4pt, belowskip=4pt} 
% \vspace{-0.1cm}
% \centering
% \includegraphics[width=0.39\textwidth]{figs/overview.png}
% \caption{\textbf{Unlike prior work, we first introduce internal visual consistency.} }
% \label{fig:intro_overview}
% \vspace{-0.25cm}
% \end{wrapfigure}
% \afterpage{\footnotetext{Code available at \url{https://github.com/pseulki/hcast}.}}

However, hierarchical classification presents a key challenge: different classification levels rely on distinct visual cues, making it a multi-task problem. For example, distinguishing \textit{Bird} from \textit{Plant} requires {global features} like feathers and leaves, whereas differentiating between fine-grained species,
such as \textit{Anna's hummingbird} and \textit{Green hermit}, depends on subtle localized details like head and neck color. This problem is further compounded when multiple objects appear in an image (Fig.~\ref{fig:intro_overview}), as different levels may attend to different objects, leading to inconsistent predictions.

To address this, existing methods focus on enforcing \textbf{semantic consistency} across levels by designing separate model components for each hierarchy level~\citep{chang2021your, chen2022label, wang2023consistency}.  While improving fine-grained accuracy in hierarchical classification, this approach often leads to \textbf{inconsistent predictions across levels}, where the model's outputs do not align with the hierarchical taxonomy. Fig.~\ref{fig:fig_intro} (b, c, d, top) illustrates such inconsistencies when training FGN~\citep{chang2021your} on the two-level hierarchy dataset BREEDS (Entity-30)\citep{data2021breeds}. For example, in (c), the coarse classifier predicts \textit{Motor Vehicle}, while the fine-grained classifier predicts \textit{Feather Boa}, demonstrating how independently optimized levels can lead to contradictions.


To understand these inconsistencies, we show Grad-CAM visualizations~\citep{selvaraju2017grad} and find that coarse and fine-grained classifiers often focus on entirely different regions (Fig.~\ref{fig:fig_intro}, bottom). For example, in case (c), the fine-grained classifier correctly attends to the \textit{feather boa}, while the coarse classifier focuses on the bicycle’s handlebars and frame, mistaking them for key features instead of capturing the broader shape of the feather boa, leading to a misclassification as \textit{Motor Vehicle}. In contrast, in the consistently correct case (Fig.~\ref{fig:fig_intro} (a)), the coarse classifier captures the bird’s shape, while the fine-grained classifier focuses on its legs, ensuring visually consistent attention across levels. We frequently observe this pattern  and provide quantitative validation in Appendix~\ref{appendix:quantitative_gradcam}.


\input{figs/intro_examples}


From this observation, we argue that hierarchical classification benefits when coarse and fine-grained classifiers maintain \textbf{visual consistency, focusing on the same object at different levels of detail}. Based on this insight, we propose a novel method that aligns their focus areas, rather than training them as separate components (Fig.~\ref{fig:comparison_prior}, right).
For instance, while the fine-grained classifier examines localized details like the \textit{beak}, \textit{wings}, and \textit{tail} to classify \textit{Green Hermit}, the coarse classifier differentiates  between \textit{birds} and \textit{plants} by integrating these details into the bird's overall \textit{body shape}.
To enforce this structured visual parsing, we propose an integrated model that progressively groups fine-grained details into coarser shapes while transferring learned features across levels. This hierarchical learning scheme effectively mitigates inconsistencies compared to prior methods, which process each level independently.


To identify and group relevant visual details, we leverage CAST~\citep{ke2024cast}, an unsupervised segmentation method that groups related pixels consistently through internal parsing without requiring segmentation labels. 
Inspired by this, we introduce Hierarchical-CAST (H-CAST), which uses fine-to-coarse semantic parsing to align classifier focus across levels.
To the best of our knowledge, our work is \textbf{the first to address internal visual consistency in hierarchical classification using unsupervised semantic segments} (Fig.~\ref{fig:intro_overview}). 
Since our method is an integrated model, if details initially captured at the fine-grained level are incorrect, it will receive negative signals (errors) during the learning process toward coarser levels. 
As training processes, the model is encouraged to capture accurate fine-grained details to improve  overall hierarchical classification performance. 

Additionally, we propose \ourloss that further enhances \textbf{semantic consistency} by ensuring predictions remain aligned with the taxonomy across levels. As a result, our method consistently produces correct predictions across all cases in Fig.~\ref{fig:fig_intro}.


First, we evaluate CLIP~\citep{ref:clip_2021} and show that even vision foundation models struggle with inconsistent hierarchical classification. To assess both accuracy and consistency, we introduce a new metric, Full-Path Accuracy (FPA), which measures the proportion of samples correctly predicted at all hierarchy levels.
Validated on standard benchmarks, our method outperforms state-of-the-art models, achieving 10+ percentage points higher FPA than ViT-based baselines on BREEDS, ensuring superior consistency and robustness. We validate its effectiveness through extensive experiments and analysis. Additionally, we show that hierarchical semantic taxonomy enhances image segmentation.

{\bf Our contributions.}
{\bf 1)} We introduce \textbf{internal visual consistency}, aligning fine-to-coarse semantic parsing with consistent visual segmentation to ensure classifiers across levels focus on coherent and related regions.
{\bf 2)} We propose a \textbf{Tree-Path KL Divergence Loss} to enforce semantic consistency across hierarchy levels.
{\bf 3)} Our method significantly outperforms ViT-based baselines, achieving +3–10\% FPA across all datasets, demonstrating superior consistency and robustness.




% \iffalse

% The goal of hierarchical classification is to predict all classes at each hierarchical level simultaneously (e.g., \textit{Ruby-throated Hummingbird} - \textit{Bird}).
% Fig.~\ref{fig:problem} provides an example of various challenges in the hierarchical classification problem. 
% For our analysis, we conduct training on the iNaturalist 2018 dataset~\citep{ref:data_iNat}, with a two-level hierarchy.
% Following the most commonly used approach for hierarchical classification~\citep{chen2018fine, chang2021your, chen2022label}, we extract features from a shared backbone (ImageNet~\citep{ref:data_imagenet}-pretrained ResNet-50~\citep{ref:resnet_cvpr2016}) and train separate classifiers to predict classes at each level.
 
% Unlike flat-level classification, hierarchical classification has multiple possible outputs.  The challenges arise when predictions at the fine and coarse levels differ (2nd and 3rd rows in Fig.~\ref{fig:problem}). 
% Even if predictions are correct at one level,  it is difficult to trust the prediction if predictions at other levels are incorrect (e.g., \textit{Ruby-throated Hummingbird} - \textit{Plant}), especially when we do not have ground truth labels at test time.
% Therefore, our focus lies in achieving consistent and accurate predictions across all levels simultaneously.

% However, predicting multiple levels of hierarchy is more challenging than predicting a single flat-level category, leading to a confrontation between coarse and fine-grained level learning~\citep{chang2021your}.
% That is, models trained to predict all hierarchical levels show degraded performance compared to the model trained to predict a single flat level of class.
% This is because hierarchical classification entails addressing multiple classification tasks concurrently.
% For instance, distinguishing between similar-looking bird species at the finest level (e.g., \textit{Anna's Hummingbird} - \textit{Ruby-throated Hummingbird}) and differentiating between birds and plants at the coarse level represent distinct tasks, each requiring attention to different regions in the image.
% This phenomenon is illustrated in Fig.~\ref{fig:comparison_prior}, where we observe that classifiers at each level often internally attend to different parts of the image.
% From this observation, we attribute performance degradation in hierarchical recognition to the inconsistency among hierarchy classifiers. 
% We seek to enhance consistency by guiding classifiers to consistently focus on the same areas, where ``\textit{bird}'' (for the coarse classifier) and ``\textit{Ruby-throated Hummingbird}'' (for the fine-level classifier) are located. 





% \textbf{Our insight} is that although the fine-level classifier and the coarse classifier may have different focal points, they are inherently connected.
% For instance, while the fine-level classifier examines aspects like the \textit{beak}, \textit{wings}, and \textit{feathers} to classify bird species, the coarse classifier can discern between birds and flowers by integrating these details into the overall \textit{body} of the bird.
% In other words, the coarse classifier should focus on the larger part formed by grouping the features attended to by the fine classifier.
% Therefore, we hypothesize that by consistently aligning the areas of focus for the fine classifier and coarse classifier, we could improve both consistency and accuracy.

% To this end, we employ the recent unsupervised image segmentation method, CAST~\citep{ke2024cast}. 
% %CAST exhibited hierarchical segmentation, transitioning from finer to coarser segments.
% CAST has demonstrated the capability to group related pixels consistently through internal parsing within images, \textit{without} segmentation labels. 
% Inspired by this, we propose {\it Hierarchical-CAST} (H-CAST), which utilizes CAST to align the focus of different levels of classifiers on the same areas for hierarchical recognition.
% Unlike previous hierarchical classification approaches that train separate models for each level~\citep{chang2021your, liu2022focus, chen2022label}, H-CAST is an integrated model where features learned at the fine-grained level are grouped and passed to the coarse level (Fig.~\ref{fig:comparison_prior}), ensuring \textbf{spatial consistency}.
% Since our method is an integrated model, if details initially captured at the fine-grained level are incorrect, it will receive negative signals (errors) during the learning process toward coarser levels. 
% As training processes, the model is encouraged to capture accurate fine-level details to improve learning at subsequent levels. 

% Additionally, we propose \ourloss to further enhance \textbf{semantic consistency} by considering label relationships across levels so that predictions at the fine-level and coarse-level align within the taxonomy.
% In Fig.~\ref{fig:problem}, we can observe that our method of improving consistency surprisingly leads to an enhancement in accuracy as well. 
% Many previously inconsistent and incorrect cases are transformed into correct classifications.

% To assess both accuracy and consistency, we evaluate our method with a new metric called Full-Path Accuracy (FPA), which measures the proportion of samples in the dataset correctly predicted at all hierarchy levels. 
% Validated on common benchmarks for hierarchical recognition, our method consistently outperforms the ViT-based baseline by more than 17-25\%p in FPA metric.  We empirically demonstrate its effectiveness through extensive experiments and analysis.  Furthermore, compared to the common segmentation learned through a flat semantic taxonomy, we demonstrate that a hierarchical semantic taxonomy also in turn improves image segmentation. 

% Our key contributions can be summarized as follows.
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
%     \item \textbf{Hierarchical-CAST (H-CAST)}: We propose H-CAST to consistently align the focus of hierarchy classifiers within the image. Our model enables the utilization of various granular segments, ensuring that focus remains on the same region while fine-detailed features transitioning to broader features at the coarse level (\textbf{spatial consistency}). This expansion of the focus region fosters a natural and consistent learning process for hierarchical recognition.
%     \item \textbf{\ourloss}: We introduce a novel loss function that considers label relationships across hierarchy levels (\textbf{semantic consistency}).
%     Our loss enforces predictions to be correct at different levels, demanding accuracy and consistency at the same time.   
%     \item These contributions combined lead to \textbf{significant improvements in both accuracy and consistency}, which we demonstrate via a new metric: Full-Path Accuracy (FPA).
% \end{itemize}

% \fi

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figs/concept_arch.png}
%   \caption{\textbf{Comparison with prior works.} Prior works~\citep{zhu2017b, yan2015hd, liu2022focus, chen2022label, chen2018fine} train separate branches for features extracted from a shared backbone to achieve hierarchical recognition, typically connecting from coarse to fine-grained levels. In contrast, our model employs a progressive learning scheme to ensure that different hierarchical granularities contribute consistently to learning in the next level, such as learning about a bird's \textcolor{mylightred}{beak} and \textcolor{mylightred}{wings} in the finer level and then combining it in the next level to learn about bird's \textcolor{myred}{body}.}
%   \label{fig:comparison_prior}
% \end{figure}



% To learn where to focus properly, previous work designs complex attention modules~\citep{liu2022focus}.
%Therefore, our goal is to enable the model to learn the distinguishing granularity features for each level without the need for a specifically designed complex attention module to determine where to look within the image.


\input{figs/fig-example_inconsistence}
       

    






==> tables/tab-ablation-architecture.tex <==
\begin{wraptable}{r}{8cm}
\vspace{-0.2cm}
\caption{\textbf{Coarse-to-Fine learning scheme achieves best overall performance.} We report the impact of hierarchical learning direction on FGVC-Aircraft.}\label{tab:ablation-arch}
\centering
\resizebox{1\linewidth}{!}
{
\begin{tabular}{c|ccccc}
\toprule
Learning Direction  & FPA & maker  & family & model & wAP                 \\ \midrule
Coarse-to-Fine      & \underline{82.01} & 93.16     & 89.92        & 84.10          & 87.50                           \\
Fine-Coarse merging & 81.76 & \underline{93.52}       & \textbf{90.31}        & \textbf{84.58}        &  \textbf{87.93}
                       \\
Fine-to-Coarse & \textbf{82.66}     & \textbf{94.27}  & \underline{90.19}  & \underline{84.40} &  \underline{87.91}
                         \\ \bottomrule
\end{tabular}
}
\vspace{-0.1cm}
\end{wraptable}



==> tables/tab-ablation-losses.tex <==
\begin{table}[tbp]
\small 
\centering
%\caption{\textbf{Loss Comparison on Living-17}}
\label{tab:ab-loss-aircraft}
\begin{minipage}{0.48\textwidth}
\raggedright
    \centering
    \caption{\textbf{Utilizing both losses yields best performance on Aircraft.}}\label{table:ablation-hstk-aircraft}
    \vspace{-3mm}
    \renewcommand{\arraystretch}{1.1} 
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{cc|ccccc}
    \toprule
    $L_{HS}$ & $L_{TK}$ & FPA & maker  & family & model & wAP                      \\ \midrule
    \xmark    & \cmark &  82.48   & 94.30  &   90.37     & 84.04      &   87.80 \\
    \cmark    & \xmark  & 82.66       & 94.27  & 90.19  & 84.40 &    87.91\\
    \cmark    & \cmark  & \textbf{83.72}  & \textbf{94.96}  & \textbf{91.39}  & \textbf{85.33} &  \textbf{88.90}\\ 
    \bottomrule
    \end{tabular}
    \end{minipage}%
\hfill
\begin{minipage}{0.48\textwidth} 
\raggedleft
    \centering
    \caption{\textbf{KL Div. loss shows best performance on Aircraft.}}\label{table:ablation-kld-aircraft}
    \vspace{-3mm}
    \renewcommand{\arraystretch}{1.1} 
    \setlength{\tabcolsep}{3pt} 
    \begin{tabular}{l|ccccc}
    \toprule
    Sem. Consis. & FPA   & maker & family & model & wAP   \\ \midrule
    Flat Consis.     & 82.87 & 94.63 & 90.94  & 84.97 & 88.51 \\
    BCE             & 82.18 & 94.21 & 90.13  & 84.88 & 88.11 \\
    KL Div. Loss         & \textbf{83.72} & \textbf{94.96} & \textbf{91.39}  & \textbf{85.33} & \textbf{88.90} \\ \bottomrule
    \end{tabular}
\end{minipage}
\vspace{-0.3cm}
\end{table}


% \begin{wraptable}{r}{8cm}
% %\vspace{-0.3cm}
% \caption{\textbf{Utilizing both losses yields best performance.} We report the effect of proposed losses on FGVC-Aircraft.}\label{table:ablation-losses-aircraft}
% \centering
% \resizebox{1\linewidth}{!}
% {
% \begin{tabular}{l|ccccc}
% \hline
% Semantic Consistency & FPA   & maker & family & model & wAP   \\ \hline
% Flat Cons. Loss      & 82.87 & 94.63 & 90.94  & 84.97 & 88.51 \\
% BCE Loss             & 82.18 & 94.21 & 90.13  & 84.88 & 88.11 \\
% KL Div. Loss         & 83.72 & 94.96 & 91.39  & 85.33 & 88.90 \\ \hline
% \end{tabular}
% }
% % \vspace{-0.2cm}
% \end{wraptable}


% \begin{table}[]
% \begin{tabular}{l|ccccc}
% \hline
% Semantic Consistency & FPA   & maker & family & model & wAP   \\ \hline
% Flat Cons. Loss      & 82.87 & 94.63 & 90.94  & 84.97 & 88.51 \\
% BCE Loss             & 82.18 & 94.21 & 90.13  & 84.88 & 88.11 \\
% KL Div. Loss         & 83.72 & 94.96 & 91.39  & 85.33 & 88.90 \\ \hline
% \end{tabular}
% \end{table}

==> tables/tab-main-breeds-living.tex <==

\begin{table}[t]
\caption{\textbf{Living-17 and Non-Living-26.} HiE~\citep{ref:hie_neurips_2023} FGN~\citep{chang2021your}, HRN~\citep{chen2022label} ...Our method demonstrates the best performance in terms of both accuracy and consistency. Compared to prior state-of-the-art methods, it shows an improvement of over 20 percentage points in the full-path accuracy metric.}\label{table:main-breeds-living}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|lcccc|ccccc|ccccc}
\toprule
     & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{Living-17 (17-34)}                                            & \multicolumn{5}{c}{Non-Living-26 (26-52)}                                          \\ \cmidrule{7-16}
             &    & Backbone             & \# Params            & Input image          & Batch size            & FPA            & Coarse         & Fine           & wAP            & TICE          & FPA            & Coarse         & Fine           & wAP            & TICE          \\ \midrule
 \multirow{4}{*}{\rotatebox{90}{Flat}} & Flat-ViT       & ViT-S            & 65.0M                & 224x224              & 256                   & 66.24          & 75.71          & 72.06          & 73.28          & 17.11         & 57.46          & 67.50          & 65.73          & 57.46          & 23.27         \\
& Flat-ViT + HiE      & ViT-S            & 65.0M                & 224x224              & 256                   & 67.59          & 75.71          & 71.35          & 72.81          & 9.88         & 59.73          & 67.50          & 65.31          & 66.04          & 13.69         \\
& Flat-CAST      & ViT-S            & 78.5M                & 224x224              & 256                   & 78.82          & 88.06          & 82.88          & 84.61          & 8.82          & 76.17          & 84.77          & 81.08          & 82.31          & 11.77         \\ 
& Flat-CAST + HiE      & ViT-S             & 78.5M                & 224x224              & 256                   & 81.59          & 88.06          & 83.24         & 84.85          & 5.18          & 79.23          & 84.77          & 81.39          & 82.51          & 6.19         \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Hierarchy}} & FGN & RN-50            & 24.8M                & 224x224              & 128                   & 63.82          & 72.59          & 68.00          & 69.53          & 12.12         & 60.81          & 69.46          & 65.77          & 67.00          & 16.46         \\
& HRN & RN-50            & 70.8M                & 224x224              & 128                   & 50.59          & 62.53          & 56.76          & 58.69          & 19.94         & 45.42          & 54.81          & 52.58          & 53.32          & 25.73         \\
& HRN & RN-50            & 70.8M                & 448x448              & 8                    & \underline{79.18}          & \underline{87.53}          &\underline{ 81.47}          & \underline{83.49}          & \underline{6.29}         & \underline{76.31}          & \underline{82.38 }         & \underline{80.15 }         & \underline{80.90 }         & \underline{9.54}         \\ \cmidrule{2-16}
& Hier-ViT         & ViT-S            & 21.7M                & 224x224              & 256                   & 74.06          & 80.94          & 74.88          & 76.90          & 10.50         & 72.04          & 73.31          & 58.39          & 70.03          & 12.45         \\
%\rowcolor{myyellow}
& Ours (H-CAST)             & ViT-S            & 26.2M                & 224x224              & 256                   & \textbf{85.12} & \textbf{90.82} & \textbf{85.24} & \textbf{87.10} & \textbf{3.19} & \textbf{82.67} & \textbf{87.89} & \textbf{83.15} & \textbf{84.73} & \textbf{5.26} \\ \cmidrule{2-16}
& \multicolumn{2}{l}{\textit{Our Gains over SOTA}}  & & & & \green{+5.94} & \green{+3.29} & \green{+3.77} & \green{+3.61} & \green{+3.10} & \green{+6.36} & \green{+5.51} & \green{+3.00} & \green{+3.83} & \green{+4.28} \\ \bottomrule
\end{tabular}
}
\end{table}
%\vspace{-0.5cm}


%\vspace{-0.5cm}


% \begin{table}[t]
% \caption{\textbf{Comparison of Methods in terms of Accuracy(\%) and Consistency Metrics(\%) on BREEDS benchmarks.}
% Our model (H-CAST) significantly outperforms Hier-ViT in both Accuracy and Consistency metrics (\underline{Our Gains}).
% }
% \label{table:main-breeds}
% \centering
% \small
% \resizebox{1\linewidth}{!}
% {
% \begin{tabular}{l|cccccccccc}
% \toprule
% \multirow{2}{*}{Method}&   \multicolumn{5}{c|}{Living-17 (17-34)}                                                                                                     & \multicolumn{5}{c}{Non-Living-26 (26-52)} \\ \cmidrule{2-11} 
%                            & FPA                       & coarse                    & fine                      & wAP                       & \multicolumn{1}{c|}{TICE}  & FPA                       & coarse                    & fine                     & wAP                       & TICE \\ \midrule                      
% Flat-ViT    & 66.24                     & 75.71                     & 72.06                     & 73.28                     & \multicolumn{1}{c|}{17.11} & 57.46                     & 65.73                     & 66.32                    & 57.46                     & 23.27                     \\
% Flat-CAST   & 78.82                     & 88.06                     & 82.88                     & 84.61                     & \multicolumn{1}{c|}{8.82}  & 76.17                     & 84.77                     & 81.08                    & 82.31                     & 11.77                     \\ \midrule
% Hier-ViT      & 74.06                     & 80.94                     & 74.88                     & 76.90                     & \multicolumn{1}{c|}{10.50} & 72.04                     & 73.31                     & 68.39                    & 70.03                     & 12.45                     \\
%  Ours          & \textbf{85.12}                     & \textbf{90.82}                     & \textbf{85.24}                     & \textbf{87.10}                     & \multicolumn{1}{c|}{\textbf{3.19}}  & \textbf{82.67}                     & \textbf{87.89}                     & \textbf{83.15}                    & \textbf{84.73}                     & \textbf{5.26}                      \\ \midrule
% \underline{Our Gains}                & \textcolor{textgreen}{\green{+1}1.06}                     & \textcolor{textgreen}{+9.88}                     & \textcolor{textgreen}{\green{+1}0.36}                     & \textcolor{textgreen}{\green{+1}0.20}                     & \multicolumn{1}{c|}{\textcolor{textgreen}{+7.31}} & \textcolor{textgreen}{\green{+1}0.63}                     & \textcolor{textgreen}{\green{+1}4.58}                     & \textcolor{textgreen}{\green{+1}4.76}                    & \textcolor{textgreen}{\green{+1}4.70}                     & \textcolor{textgreen}{+7.19}                     \\ \midrule
%                & \multicolumn{5}{c}{Entity-13 (13-130)}                                                                                                     & \multicolumn{5}{c}{Entity-30 (30-120)}                                                                                                   \\ \midrule
% Flat-ViT    & 64.22                     & 76.28                     & 76.06                     & 76.08                     & \multicolumn{1}{c|}{21.33} & 66.93                     & 76.47                     & 74.35                    & 74.77                     & 18.75                     \\
%  Flat-CAST   & 78.63                     & 87.80                     & 83.72                     & 84.09                     & \multicolumn{1}{c|}{10.65} & 82.67                     & 87.89                     & 83.15                    & 84.73                     & 5.26                      \\ \midrule
% Hier-ViT      & 74.63                     & 86.95                     & 75.39                     & 77.70                     & \multicolumn{1}{c|}{5.19}  & 73.01                     & 81.38                     & 74.10                    & 74.76                     & 11.61                     \\
% Ours          & \textbf{85.68}                     & \textbf{93.42}                     & \textbf{86.15}                     & \textbf{87.60}                     & \multicolumn{1}{c|}{\textbf{1.69}}  & \textbf{84.83}                     & \textbf{90.23}                     & \textbf{85.45}                    & \textbf{85.88}                     & \textbf{2.57}                      \\ \midrule
% \underline{Our Gains} & \textcolor{textgreen}{\green{+1}1.05} & \textcolor{textgreen}{+6.47}  & \textcolor{textgreen}{\green{+1}0.76} & \textcolor{textgreen}{+9.90} & \multicolumn{1}{c|}{\textcolor{textgreen}{+3.50}}  & \textcolor{textgreen}{\green{+1}1.82}  & \textcolor{textgreen}{+8.85}   & \textcolor{textgreen}{\green{+1}1.35}   & \textcolor{textgreen}{\green{+1}1.12} & \textcolor{textgreen}{+9.04} \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}






% \begin{tabular}{ll|ccccc||ccccc}
% \toprule
% \multicolumn{2}{c|}{\multirow{3}{*}{Method}} & \multicolumn{5}{c||}{Living-17 (17-34)}                                                             & \multicolumn{5}{c}{Non-Living-26 (26-52)}                                           \\ \cline{3-12} 
% \multicolumn{2}{c|}{}                        & \multicolumn{3}{c|}{Accuracy}                           & \multicolumn{2}{c||}{Consistency} & \multicolumn{3}{c|}{Accuracy}             & \multicolumn{2}{c}{Consistency} \\ \cline{3-12} 
% \multicolumn{2}{c|}{}                        & coarse($\uparrow$)               & fine($\uparrow$)  & \multicolumn{1}{c|}{wAP($\uparrow$)}  & FPA($\uparrow$) & TICE($\downarrow$)                      & coarse($\uparrow$) & fine($\uparrow$)  & \multicolumn{1}{c|}{wAP($\uparrow$)} & FPA($\uparrow$) & TICE($\downarrow$)               \\ \midrule
% \multirow{2}{*}{Flat}      & ViT-Flat    &   75.71            & 72.06   & \multicolumn{1}{c|}{73.28}    &  66.24  & 17.11                 &  67.50      & 65.73   & \multicolumn{1}{c|}{66.32}    &    57.46            &  23.27              \\
%                              & CAST-Flat   &   88.06                   & 82.88   & \multicolumn{1}{c|}{84.61}    &   79.82 &   8.82                   &  84.77   & 81.08   & \multicolumn{1}{c|}{82.31}    &    76.17         &   11.77         \\ \midrule
% \multirow{2}{*}{Hierarchy}   & Hier-ViT      & 80.94                & 74.88 &  \multicolumn{1}{c|}{76.90}    &  74.06        &   10.50       & 73.31  & 68.39 & \multicolumn{1}{c|}{70.03}    &  72.04      &    12.45        \\
%                              & H-CAST          & \textbf{90.82}                & \textbf{85.24} & \multicolumn{1}{c|}{\textbf{87.10}}    &   \textbf{85.12}         &   \textbf{3.19}             & \textbf{87.89}  & \textbf{83.15} & \multicolumn{1}{c|}{\textbf{84.73}}    &   \textbf{82.67}             &     \textbf{5.26}           \\ \midrule \midrule
%                              &               & \multicolumn{5}{c||}{Entity-13 (13-130)}                                                             & \multicolumn{5}{c}{Entity-30 (30-120)}                                               \\ \midrule
% \multirow{2}{*}{Flat}      & ViT-Flat    &     76.28                 & 76.06   & \multicolumn{1}{c|}{76.08}    &    64.22             &    21.23            &  76.47      & 74.35   & \multicolumn{1}{c|}{74.77}    &        66.93        &     18.75           \\
%                              & CAST-Flat   & 87.80 & 83.72   & \multicolumn{1}{c|}{84.09}    &  78.63               &   10.65             &  85.89      & 83.32
%    & \multicolumn{1}{c|}{83.83}    & 78.72               &   9.33             \\ \midrule
% \multirow{2}{*}{Hierarchy}   & Hier-ViT      & 86.95                & 75.39 & \multicolumn{1}{c|}{77.70}    &   74.63              &   5.19         & 81.38  & 74.10 & \multicolumn{1}{c|}{74.76}    &   73.01        &    11.61      \\
%                              & H-CAST          & \textbf{93.42}                & \textbf{86.15} & \multicolumn{1}{c|}{\textbf{87.60}}    &   \textbf{85.68}        &  \textbf{1.69}          & \textbf{90.23}  & \textbf{85.45} & \multicolumn{1}{c|}{\textbf{85.88}}    &     \textbf{84.83}     &    \textbf{2.57}      \\ \bottomrule
% \end{tabular}
% }

% \begin{table}[t]
% \centering
% \small
% \resizebox{0.9\linewidth}{!}
% {
% \begin{tabular}{ll|ccccc|ccccc}
% \midrule
% \multicolumn{2}{c|}{\multirow{3}{*}{Method}} & \multicolumn{5}{c|}{Entity-13}                                               & \multicolumn{5}{c}{Entity-30}                                               \\ \cline{3-12} 
% \multicolumn{2}{c|}{}                        & \multicolumn{3}{c|}{Accuracy}             & \multicolumn{2}{c|}{Consistency} & \multicolumn{3}{c|}{Accuracy}             & \multicolumn{2}{c}{Consistency} \\ \cline{3-12} 
% \multicolumn{2}{c|}{}                        & coarse & fine  & \multicolumn{1}{c|}{wAP} & TICE            & FPA           & coarse & fine  & \multicolumn{1}{c|}{wAP} & TICE           & FPA           \\ \midrule
% \multirow{2}{*}{Flat}      & ViT-Flat    &        & ing   & \multicolumn{1}{c|}{}    &                 &                &        & ing   & \multicolumn{1}{c|}{}    &                &                \\
%                              & CAST-Flat   &        & ing   & \multicolumn{1}{c|}{}    &                 &                &        & ing   & \multicolumn{1}{c|}{}    &                &                \\ \midrule
% \multirow{2}{*}{Hierarchy}   & Hier-ViT      & 86.95  & 75.39 & \multicolumn{1}{c|}{}    &                 &                & 81.38  & 74.10 & \multicolumn{1}{c|}{}    &                &                \\
%                              & H-CAST          & 93.42  & 86.15 & \multicolumn{1}{c|}{}    &                 &                & 90.23  & 85.45 & \multicolumn{1}{c|}{}    &                &                \\ \midrule
% \end{tabular}
% }
% \end{table}

==> tables/tab-segmentation.tex <==
\begin{table} %{r}{8cm}
\textbf{\large Region accuracy on BREEDS with ground truth segmentation}
\centering
\resizebox{0.85\linewidth}{!}
{
\begin{tabular}{l|cccc}
\toprule
region mIOU   & Living-17 & Non-Living-26 & Entity-30 & Entity-13 \\ \midrule
CAST       & 31.52     & 21.86         & \textbf{23.30}  & 14.41          \\
H-CAST     & \textbf{32.83}     & \textbf{22.12}     & 22.08     & \textbf{16.19}          \\ \bottomrule
\end{tabular}
\vspace{2cm}
}
\end{table}
\vspace{2cm}


% \caption{\textbf{Using taxonomy helps in segmenting object parts on BREEDS with ImageNet-S.} To quantitatively verify its effectiveness in segmentation, we measured the region mIOU of Fine-level objects for samples whose segmentation ground truth data from can be obtained from ImageNet-S.
% Both CAST and H-CAST utilize the last level segments. Since H-CAST uses coarse-level supervision for the last level segments, H-CAST can underperform compared to CAST, which employs fine-level supervision. Nevertheless, H-CAST outperforms CAST in most datasets, demonstrating that utilizing additional taxonomy is effective not only for recognition but also for segmentation.}
